THE TOOLS AND MONTE CARLO WORKING GROUP Summary Report from the Les Houches 2009 Workshop on TeV Colliders

This is the summary and introduction to the proceedings contributions for the Les Houches 2009 "Tools and Monte Carlo" working group.

==> lhdefs.tex <==
%%% To work with JHEP.cls, (x)color.sty needs this work-around:
\usepackage{xcolor}
\makeatletter
\let\default@color\current@color
\makeatother

%%% I'm not sure if we really want to format URLs \smaller ...
\usepackage{url}
% \makeatletter
% \def\url@smallerstyle{%
%   \@ifundefined{selectfont}{\def\UrlFont{\smaller}}{\def\UrlFont{\smaller}}}
% \makeatother
% \urlstyle{smaller}

%% Auto bold math in bold environments
\makeatletter
\g@addto@macro\bfseries{\boldmath}
\makeatother

\IfFileExists{microtype.sty}{%
  \RequirePackage{microtype}%
  %\RequirePackage[tracking=true]{microtype}%
  %\UseMicrotypeSet[tracking]{smallcaps}%
  %\SetTracking{encoding=*,shape=sc}{30}
}{}


%%% A very visible way of displaying TODOs:
\definecolor{todoboxcolor}{rgb}{1.0,0.6,0.6}
\newcommand{\TODO}[1]{\par\medskip \noindent%
\colorbox{todoboxcolor}{TODO: \parbox[t]{6.5cm}{#1}}%
\medskip\par}

\definecolor{todoneboxcolor}{rgb}{1.0,0.9,0.9}
\newcommand{\TODONE}[1]{\par\medskip \noindent%
\colorbox{todoneboxcolor}{TODONE?: \parbox[t]{6.5cm}{#1}}%
\medskip\par}

\newcommand{\xparagraph}[1]{\par\vspace{2mm}\noindent\emph{#1}\quad}
\newcommand\centerAlign[1]{%
   \raisebox{-0.5\height}{#1}%
}

\setlength{\parindent}{1em}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\DeclareMathOperator{\det}{det}

\newcommand{\EqRef}[1]{equation~\eqref{#1}\xspace}
\newcommand{\SecRef}[1]{section~\ref{#1}\xspace}
\newcommand{\TabRef}[1]{Table~\ref{#1}\xspace}
\newcommand{\FigRef}[1]{Figure~\ref{#1}\xspace}
\newcommand{\TabsRef}[1]{Tables~\ref{#1}\xspace}
\newcommand{\FigsRef}[1]{Figures~\ref{#1}\xspace}

\newcommand{\DeltaOf}[1]{\ensuremath{\Delta\mspace{0.75mu}#1}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\nCr}[2]{\ensuremath{\parenths{\colvec{#1 \\ #2}}}\xspace}
\newcommand{\alphaS}{\ensuremath{\alpha_\text{s}}\xspace}
\newcommand{\sqrts}{\ensuremath{\sqrt{s}}\xspace}
\newcommand{\pTmin}{\ensuremath{{p_{\perp}^\text{\:min}}}\xspace}
\newcommand{\pTlead}{\ensuremath{{p_{\perp}^\text{\:lead}}}\xspace}
\newcommand{\pTleadmin}{\ensuremath{{p_{\perp}^\text{\:lead, min}}}\xspace}
\newcommand{\pTleadmax}{\ensuremath{{p_{\perp}^\text{\:lead, max}}}\xspace}
\newcommand{\LambdaQCD}{\ensuremath{\Lambda_\text{QCD}}\xspace}
\newcommand{\ofOrder}[1]{\ensuremath{\mathcal{O}(#1)}\xspace}
\newcommand{\order}[1]{\ensuremath{\mathcal{O}(#1)}\xspace}
\newcommand{\kbd}[1]{{\smaller{\texttt{#1}}}}


\def\PARJ#1{\ensuremath{\text{PARJ(#1)}}}
\def\PARP#1{\ensuremath{\text{PARP(#1)}}}
\def\MSTJ#1{\ensuremath{\text{MSTJ(#1)}}}


%%% Some names, to use a consistent spelling throughout the document:
\def\aleph{ALEPH\xspace}
\def\delphi{DELPHI\xspace}
\def\tasso{TASSO\xspace}
\def\opal{OPAL\xspace}
\def\lthree{L3\xspace}
\def\cdf{CDF\xspace}
\def\dzero{D\O\xspace}
\def\ATLAS{ATLAS\xspace}
\def\cms{CMS\xspace}
\def\atlas{ATLAS\xspace}

\def\lep{LEP\xspace}
\def\lepi{LEP~1\xspace}
\def\lhc{LHC\xspace}
\def\tevatron{Tevatron\xspace}
\def\rhic{RHIC\xspace}
\def\hera{HERA\xspace}
\def\sld{SLD\xspace}

\def\fnal{FNAL\xspace}
\def\cern{CERN\xspace}

\def\mcnet{MCnet\xspace}
\def\pdg{PDG\xspace}

\def\runi{Run-\textsmaller{I}\xspace}
\def\runii{Run-\textsmaller{II}\xspace}
\def\runiia{Run-\textsmaller{II}a\xspace}
\def\runiib{Run-\textsmaller{II}b\xspace}

\def\Cpp{C\raisebox{0.2ex}{\smaller++}\xspace}

\def\fortran{Fortran\xspace}
\def\pythia{Pythia\xspace}
\def\phojet{Phojet\xspace}
\def\pythiasix{Pythia~6\xspace}
\def\pythiaeight{Pythia~8\xspace}
\def\herwig{Herwig\xspace}
\def\herwigsix{Herwig~6\xspace}
\def\herwigpp{Herwig\raisebox{0.1ex}{\smaller++}\xspace}
\def\sherpa{Sherpa\xspace}
\def\alpgen{AlpGen\xspace}
\def\charybdis{Charybdis\xspace}
\def\jimmy{Jimmy\xspace}
\def\rivet{Rivet\xspace}
\def\rivetgun{Rivetgun\xspace}
\def\professor{Professor\xspace}
\def\fastjet{FastJet\xspace}
\def\hepmc{HepMC\xspace}
\def\agile{AGILe\xspace}
\def\hztool{HZTool\xspace}
\def\numpy{NumPy\xspace}
\def\scipy{SciPy\xspace}
\def\minuit{Minuit\xspace}
\def\pyminuit{PyMinuit\xspace}
\def\python{Python\xspace}

\def\jade{Jade\xspace}
\def\durham{Durham\xspace}

\def\gof{GoF\xspace}

\def\wg{$W\gamma$ }
\def\baur{\textsc{Wgamma\_NLO }}
%\def\pythia{\textsc{Pythia }} 
\def\ptg{$p_{T}^{\gamma}$ } 

\newcommand{\pt}{\ensuremath{p_T}\xspace}
\newcommand{\et}{\ensuremath{E_T}\xspace}
\newcommand{\kt}{\ensuremath{k_\perp}\xspace}
\newcommand{\pT}{\ensuremath{p_T}\xspace}
\newcommand{\kT}{\ensuremath{k_\perp}\xspace}

\newcommand{\Z}  {\mbox{$Z/\gamma^*$}}
\newcommand{\z}  {\mbox{$Z/\gamma^*$}}
\newcommand{\w}  {\mbox{$W$}}
\newcommand{\W}  {\mbox{$W$}}
\newcommand{\zee}  {\mbox{$Z/\gamma^* \rightarrow e^+ e^-$}}
\newcommand{\zmm}  {\mbox{$Z/\gamma^* \rightarrow \mu^+ß \mu^-$}}

\newcommand{\ttbar}  {\mbox{$t\bar{t}$}\xspace}
\newcommand{\bbbar}  {\mbox{$b\bar{b}$}\xspace}
\newcommand{\ttH}  {\mbox{$t\bar{t}H$}\xspace}

\newcommand{\at}  {\mbox{$a_{T}$}}
\newcommand{\dr}  {\mbox{$\Delta R$}}

\newcommand{\perugia}  {{$Perugia$}}
\newcommand{\cteq}  {{CTEQ}}


\newcommand{\program}[1]{\textsf{#1}}


\newcommand{\SUB}[2]{\ensuremath{#1_{\mathrm{#2}}}}
\newcommand{\pThat}{\SUB{\hat{p}}{T}}
\newcommand{\yscale}{\SUB{y}{scale}}
\newcommand{\mj}{\SUB{m}{jet}}
\newcommand{\nvtx}{\SUB{N}{vtx}}
\newcommand{\HS}[1]{\SUB{#1}{HS}}
\newcommand{\PU}[1]{\SUB{#1}{HS+PU}}

\newcommand{\abs}[1]{\left| #1\right|}
\newcommand{\rbr}[1]{\left( #1\right)}
\newcommand{\abr}[1]{\langle #1\rangle}
\newcommand{\cbr}[1]{\left\{ #1\right\}}
\newcommand{\sbr}[1]{\left[ #1\right]}
\newcommand{\done}{{\rm d}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\dst}{\displaystyle}
\newcommand{\sst}{\scriptstyle}
\newcommand\POWHEG{{\tt P\scalebox{0.9}{OWHEG}}\xspace}
\newcommand\POWHEGBOX{{\tt P\scalebox{0.9}{OWHEG} B\scalebox{0.9}{OX}}\xspace}
\newcommand\MCatNLO{{\tt M\scalebox{0.9}{C}@N\scalebox{0.9}{LO}}\xspace}
\newcommand\ARIADNE{{\tt A\scalebox{0.9}{RIADNE}}\xspace}
\newcommand\ADICIC{{\tt A\scalebox{0.9}{DICIC}++}\xspace}
\newcommand\AMEGIC{{\tt A\scalebox{0.9}{MEGIC}++}\xspace}
\newcommand\Comix{{\tt Comix}\xspace}
\newcommand\HNNLO{{\tt H\scalebox{0.9}{NNLO}}\xspace}
\newcommand\MGME{{\tt M\scalebox{0.9}{AD}G\scalebox{0.9}{RAPH/}M\scalebox{0.9}{AD}E\scalebox{0.9}{VENT}}\xspace}
\newcommand\qt{q_{\sss\rm T}}
\newcommand\sss{\mathchoice%
{\displaystyle}%
{\scriptstyle}%
{\scriptscriptstyle}%
{\scriptscriptstyle}%
}


\newcommand{\ttt}[1]{\texttt{#1}}
\newcommand{\snumentry}[2]{
\begin{minipage}[t]{1.2cm}\flushright\ttt{#1}\end{minipage}
\hspace{2mm}:
%
\begin{minipage}[t]{11cm}\noindent
#2\end{minipage}\\[1mm]
}
\newcommand{\numentry}[2]{
\begin{minipage}[t]{1.2cm}\flushright\texttt{#1}\end{minipage}
\hspace{2mm}:
\begin{minipage}[t]{11cm}\noindent
#2\end{minipage}\\[1mm]
}
\def\citeres#1{\mbox{Refs.~\cite{#1}}}
\def\refse#1{\mbox{Sect.~\ref{#1}}}
\def\citere#1{\mbox{Ref.~\cite{#1}}}
\newcommand{\dummy}{}
\newcommand{\leaveout}[1]{\renewcommand{\dummy}{#1}}


==> tables/plateudefs.tex <==
\begin{table}[htbp]
\begin{center}
  \begin{tabular}{l||c|c}
      \toprule
      $\sqrt{s}/\TeV$ & \pTleadmin/\GeV & \pTleadmax/\GeV \\
      \midrule
      0.2  & 10 & 30 \\
      0.63 & & \\
      0.9  & 25 & 80 \\
      1.8  & 30 & 80 \\
      1.96 & 35 & 90 \\
      2.36 & & \\
      5.0  & & \\
      7.0  & 40 & 120 \\
      10.0 & 40 & 150 \\
      14.0 & 40 & 160 \\
      \bottomrule
  \end{tabular}
  \caption{Definition of plateau regions (\pTlead) used in the extrapolation study.}
  \label{tab:plateaudefs}
\end{center}
\end{table}


==> tables/table_weights_JIMMY_LOSTAR.tex <==
\begin{table}[htbp]
\begin{center}
  \begin{tabular}{lc}
    \hline
    Observable                                                    & Weight \\
    \hline
    \textit{CDF run \textsc{I} underlying event in dijet events}\cite{Affolder:2001xt}:            &    \\
    $N_\text{ch}$ density vs leading jet $p_\perp$ (transverse), JET20 &  1 \\
    $\sum p_\perp$ density vs leading jet $p_\perp$ (transverse), JET20       &  1 \\
    $p_\perp$ distribution (transverse), leading $p_\perp > \text{5}{\GeV}$  &  1 \\
    \hline
    \textit{CDF run \textsc{I} underlying event in} MINMAX-cones\cite{Acosta:2004wqa}: & \\ 
    $\langle p_\perp^\mathrm{max} \rangle$ vs. $E_\perp^\mathrm{lead}$ at $\sqrt{s}$ = 1800 GeV & 1 \\
    $\langle p_\perp^\mathrm{min} \rangle$ vs. $E_\perp^\mathrm{lead}$ at $\sqrt{s}$ = 1800 GeV & 1 \\
    $\langle p_\perp^\mathrm{diff} \rangle$ vs. $E_\perp^\mathrm{lead}$ at $\sqrt{s}$ = 1800 GeV & 1 \\
    $N_\mathrm{max}$ vs. $E_\perp^\mathrm{lead}$ at $\sqrt{s}$ = 1800 GeV & 1 \\
    $N_\mathrm{min}$ vs. $E_\perp^\mathrm{lead}$ at $\sqrt{s}$ = 1800 GeV & 1 \\
    Swiss Cheese $p_\perp^\mathrm{sum}$ vs. $E_\perp^\mathrm{lead}$ (for removal of 2 jets) at $\sqrt{s}$ = 1800 GeV & 1 \\
    $\langle p_\perp^\mathrm{max} \rangle$ vs. $E_\perp^\mathrm{lead}$ at $\sqrt{s}$ = 630 GeV & 1 \\
    $\langle p_\perp^\mathrm{min} \rangle$ vs. $E_\perp^\mathrm{lead}$ at $\sqrt{s}$ = 630 GeV & 1 \\
    $\langle p_\perp^\mathrm{diff} \rangle$ vs. $E_\perp^\mathrm{lead}$ at $\sqrt{s}$ = 630 GeV & 1 \\
    Swiss Cheese $p_\perp^\mathrm{sum}$ vs. $E_\perp^\mathrm{lead}$ (for removal of 2 jets) at $\sqrt{s}$ = 630 GeV & 1 \\
    \hline
    \textit{CDF run \textsc{II} underlying event in leading jet events}\cite{cdf-leadingjet}:          &    \\
    $N_\text{ch}$ density vs leading jet $p_\perp$ (transverse)           &  1 \\
    $N_\text{ch}$ density vs leading jet $p_\perp$ (transMAX)             &  1 \\
    $N_\text{ch}$ density vs leading jet $p_\perp$ (transMIN)             &  1 \\
    $N_\text{ch}$ density vs leading jet $p_\perp$ (transDIF)             &  1 \\
    $\sum p_\perp$ density vs leading jet $p_\perp$ (transverse)              &  1 \\
    $\sum p_\perp$ density vs leading jet $p_\perp$ (transMAX)                &  1 \\
    $\sum p_\perp$ density vs leading jet $p_\perp$ (transMIN)                &  1 \\
    $\sum p_\perp$ density vs leading jet $p_\perp$ (transDIF)                &  1 \\
    \hline
    \textit{D0 dijet angular correlations}\cite{Abazov:2004hm}:                        &    \\
    dijet azimuthal angle, $p_\perp^\text{max} \in \text{[75, 100]}{\GeV}$   &  1 \\
    dijet azimuthal angle, $p_\perp^\text{max} \in \text{[100, 130]}{\GeV}$  &  1 \\
    dijet azimuthal angle, $p_\perp^\text{max} \in \text{[130, 180]}{\GeV}$  &  1 \\
    dijet azimuthal angle, $p_\perp^\text{max} > \text{180}{\GeV}$           &  1 \\
    \hline
  \end{tabular}
  \samepage
  \caption{Observables and weights used for the LO$^*$ tuning of JIMMY with Professor}
  \label{tab:obsweights}
\end{center}
\end{table}


==> tuning-errorbands/images/Makefile <==
PLOTS = CDF_2008_LEADINGJETS_d01-x01-y01.pdf CHI2PROFILE_MEAN.pdf \
       CHI2PROFILE_SPREAD.pdf CHI2DIST.pdf 	
#FULLRANGEPLOTS = CDF_2002_S4796047_d01-x01-y01.pdf CDF_2002_S4796047_d02-x01-y01.pdf

all: $(PLOTS) $(FULLRANGEPLOTS)

$(PLOTS): %.pdf: %.dat
	make-plots --cm --pdf $<

#$(FULLRANGEPLOTS): %.pdf: %.dat
	#make-plots --cm --pdf --full-range $<


